Digital Twin-Assisted Data-Driven Optimization for Reliable Edge Caching in Wireless Networks

Optimizing edge caching is crucial for the advancement of next-generation (nextG) wireless networks, ensuring high-speed and low-latency services for mobile users. Existing data-driven optimization approaches often lack awareness of the distribution of random data variables and focus solely on optimizing cache hit rates, neglecting potential reliability concerns, such as base station overload and unbalanced cache issues. This oversight can result in system crashes and degraded user experience. To bridge this gap, we introduce a novel digital twin-assisted optimization framework, called D-REC, which integrates reinforcement learning (RL) with diverse intervention modules to ensure reliable caching in nextG wireless networks. We first develop a joint vertical and horizontal twinning approach to efficiently create network digital twins, which are then employed by D-REC as RL optimizers and safeguards, providing ample datasets for training and predictive evaluation of our cache replacement policy. By incorporating reliability modules into a constrained Markov decision process, D-REC can adaptively adjust actions, rewards, and states to comply with advantageous constraints, minimizing the risk of network failures. Theoretical analysis demonstrates comparable convergence rates between D-REC and vanilla data-driven methods without compromising caching performance. Extensive experiments validate that D-REC outperforms conventional approaches in cache hit rate and load balancing while effectively enforcing predetermined reliability intervention modules.

==> macros.tex <==

%
% The name of this file is ``macros.tex''
%

%
% TEX defaults
%
%
% frame 6.5 * 9
\textwidth 6.5in
\textheight 9in

% left/right margins
\oddsidemargin 0pt
\evensidemargin 0pt
\marginparwidth 1in
\marginparsep 0pt

% top margin
\topmargin -25pt
\headheight 10pt
\headsep 30pt
% \topskip 0pt

% foot margin
%\footheight 0pt
\footskip 27pt


% macros for commonly used special fonts
\newcommand{\IE}{{\it i.e.,}\ }
\newcommand{\EG}{{\it e.g.,}\ }
% single/double spacing
%\newcommand{\SS}{\renewcommand{\baselinestretch}{1}\large\normalsize}
\newcommand{\DS}{\renewcommand{\baselinestretch}{1.6}\large\normalsize}
% reduce the space between lines
\newcommand{\Tight}{\renewcommand{\baselinestretch}{0.9}\large\normalsize}
\newcommand{\HalfTight}{\renewcommand{\baselinestretch}{0.95}\large\normalsize}
\newcommand{\MinorTight}{\renewcommand{\baselinestretch}{0.975}\large\normalsize}
% Page title (primarily for foils)
% (this was called \HH}
\newcommand{\PageTitle}[1]{{\newpage \begin{center}{\LARGE {\bf {#1}} } \end{center} } }

% remove spaces around section headers
%\newcommand{\Section}[1]{\vspace{-3ex}\section{#1}\vspace{-2ex}}
\newcommand{\Subsection}[1]{\vspace{-2ex}\subsection{#1}\vspace{-1ex}}
\newcommand{\Subsubsection}[1]{\vspace{-2ex}\subsubsection{#1}\vspace{-1ex}}

% go forward n lines (negative for backward move)
\newcommand{\VLine}[1]{\vspace{#1ex}}
% itemize and enumerate without spaces around/between items
\newenvironment{TightItem}{\vspace{-2ex}\begin{itemize}
  \setlength{\itemsep}{-0ex}}{\end{itemize}\vspace{-1ex}}
\newenvironment{TightEnum}{\vspace{-2ex}\begin{enumerate}
  \setlength{\itemsep}{-0ex}}{\end{enumerate}\vspace{-1ex}}
\newenvironment{TightDesc}{\vspace{-1ex}\begin{description}
  \setlength{\itemsep}{-0ex}}{\end{description}\vspace{-1ex}}
% set the page number (to the first argument)
\newcommand{\SetPageNo}[1]{\countdef\pageno=0 \pageno=#1}
% things to do
\newenvironment{Todo}{\begin{large}\begin{bf}********** things to do
    ********** \\}{\\ **********\end{bf}\end{large}}
% for discussion
\newenvironment{Discuss}{\begin{large}\begin{em}**********
    things to be discussed ********** \\}{\\ **********\end{em}\end{large}}
% set the paragraph identation and separation


% the foil environment
\newenvironment{Foil}{\begin{document}\begin{LARGE}\begin{sf}
    }{\end{sf}\end{LARGE}\end{document}}
    % NOTE: ``}'' must be in the 2nd line
% foil page title
\newcommand{\Title}[1]{\newpage \center{\huge {\sf #1}} \flushleft
    \vspace{1ex}}

% set the paragraph identation and separation
\parindent 0.2in
\setlength{\parskip}{1ex}

% set text width
\textwidth = 6.75in

% set the formula separation
\setlength{\topsep}{0in}

% set indentation for formulas:
% \setlength{\mathindent}{3ex}

% set left margin
\setlength{\oddsidemargin}{-.1in}




==> response.tex <==
\section*{Response to Reviewers}

\noindent Dear Reviewers,\\

\noindent On behalf of the authors, as the corresponding author, I would like to thank you for your thoughtful comments on the initial version of the manuscript, which was submitted to 2024 IEEE JSAC Special Issue on Advanced Optimization Theory and Algorithms for Next Generation Wireless Communication Networks entitled “Digital Twin-Assisted Data-Driven Optimization for Reliable Edge Caching in Wireless Networks” (Manuscript ID: 1570979578). We believe that, in responding to your comments, we have significantly improved the quality of the paper. We carefully reviewed the paper considering your comments and revised the paper accordingly. New/changed material is highlighted in the new version so that you can locate it easily. We hope that you find the changes satisfactory and the revised manuscript successfully addresses your
questions and comments. The changes we made to the paper in response to each of your comments are detailed on the following pages.\\

\noindent Sincerely yours.

\noindent Zifan Zhang

\noindent E-mail: zzhang66@ncsu.edu

\newpage

\subsection*{Response to Reviewer A}
\noindent \textbf{Comment 1}

\noindent \textit{The work assumes all the caching slots have the same space and all the cache units require the same amount of space. Please comment on what if these conditions are not true.}

\noindent \textbf{Response}

\noindent \\


\noindent \textbf{Comment 2}

\noindent \textit{On page 4, "clusters are based on an attribute sequence of BSs ${g, k, \beta, \tau}$, which represents their geological distances, capacity of backhaul links, coverage area overlaps, and similarity of frequency of occurrence distribution, respectively" --  The first two attributes are relatively straightforward. It is better to clarify how "coverage area overlap" and "similarity of frequency of occurrence distribution" are defined.}

\noindent \textbf{Response}

\noindent \\

\noindent \textbf{Comment 3}

\noindent \textit{On page 5, Algorithm 1, "Require: ... C clusters, N BSs": does the algorithm requires only "the number of clusters C" and "the number of BSs N" or additional information of the clusters and BSs?}

\noindent \textbf{Response}

\noindent \\

\noindent \textbf{Comment 4}

\noindent \textit{In a figure with multiple subfigures, each subfigure should have its own x- and y-labels.}

\noindent \textbf{Response}

\noindent \\





\subsection*{Response to Reviewer B}

\noindent \textbf{Comment 1}

\noindent \textit{The introduction of the article states that the heterogeneity, randomness, and variability of user device preferences lead to the decreased effectiveness of traditional caching optimization methods. However, in Section II A, all user request frequencies follow a uniform Zipf distribution, and the heterogeneity and variability of requests are not reflected, which contradicts the research motivation of this article.}

\noindent \textbf{Response}

\noindent \\


\noindent \textbf{Comment 2}

\noindent \textit{The proposed solution based on RL for the formalized problem established in this article appears to be a generic description of RL without specific relevance to the content of the article.}

\noindent \textbf{Response}

\noindent \\

\noindent \textbf{Comment 3}

\noindent \textit{The organization structure of the article is not sufficiently clear and needs adjustments to improve its clarity and logical coherence. In Section II, it first introduces the modeling of cache replacement issues, followed by the presentation of digital twins and relevant reliable reinforcement learning works. The logical sequence of these parts is unclear.}

\noindent \textbf{Response}

\noindent \\

\noindent \textbf{Comment 4}

\noindent \textit{In Section III, dynamic connection segmentation (DCS) is used to cluster BSs to create the DT framework. Although the authors discuss the significance of this step in subsequent subsections, it is necessary to explain its purpose here to help readers better understand the core ideas and operational procedures of this method.}

\noindent \textbf{Response}

\noindent \\

\noindent \textbf{Comment 5}

\noindent \textit{The main research objective of this article is to optimize edge caching, but it lacks discussion on the latest relevant research on edge caching.}

\noindent \textbf{Response}

\noindent \\





\subsection*{Response to Reviewer C}

\noindent \textbf{Comment 1}

\noindent \textit{Can authors write down the motivation of this manuscript in the form of a list?}

\noindent \textbf{Response}

\noindent \\


\noindent \textbf{Comment 2}

\noindent \textit{The contributions are summarized insufficiently.}

\noindent \textbf{Response}

\noindent \\

\noindent \textbf{Comment 3}

\noindent \textit{Some of the figures in this manuscript occupy too much space, so it is suggested to arrange them reasonably, for example, the Fig.7 and Fig.11.}

\noindent \textbf{Response}

\noindent \\

\noindent \textbf{Comment 4}

\noindent \textit{The approaches are theoretical and should be more practical to show the usefulness of the approach for the optimizing edge caching. But in this manuscript, this part is not enough. Can the authors do some further work on this problem?}

\noindent \textbf{Response}

\noindent 


